Evaluating Models of Robust Word Recognition with Serial Reproduction

Spoken communication occurs in a "noisy channel" characterized by high levels of environmental noise, variability within and between speakers, and lexical and syntactic ambiguity. Given these properties of the received linguistic input, robust spoken word recognition -- and language processing more generally -- relies heavily on listeners' prior knowledge to evaluate whether candidate interpretations of that input are more or less likely. Here we compare several broad-coverage probabilistic generative language models in their ability to capture human linguistic expectations. Serial reproduction, an experimental paradigm where spoken utterances are reproduced by successive participants similar to the children's game of "Telephone," is used to elicit a sample that reflects the linguistic expectations of English-speaking adults. When we evaluate a suite of probabilistic generative language models against the yielded chains of utterances, we find that those models that make use of abstract representations of preceding linguistic context (i.e., phrase structure) best predict the changes made by people in the course of serial reproduction. A logistic regression model predicting which words in an utterance are most likely to be lost or changed in the course of spoken transmission corroborates this result. We interpret these findings in light of research highlighting the interaction of memory-based constraints and representations in language processing.

==> Telephone - Cognition revision 3-2/includes/structureTests_lm.tex <==
%latex.default(rdf, file = file, title = "", table.env = FALSE,     booktabs = TRUE, ...)%
\begin{table}[t]
\caption{A mixed-effects linear regression examining average per-word surprisal estimates (negative log probability under a model) across 9 language models as a function of 1) whether the model uses an abstract representation of the preceding context to inform expectations and 2) the dataset used to fit the model.\label{tab:structure_lm}} 
\begin{center}
\begin{tabular}{lllll}
\toprule
Fixed Effects&&&&\tabularnewline
\multicolumn{1}{l}{}&\multicolumn{1}{c}{Coef $\beta$}&\multicolumn{1}{c}{SE($\beta$)}&\multicolumn{1}{c}{\textit{t} value}&\multicolumn{1}{c}{$p$}\tabularnewline
\midrule
(Intercept)&2.3362&0.0272&85.81&\textbf{\textless .0001}\tabularnewline
generation&0.001&0.0025&0.38&0.7\tabularnewline
abstract structure: used&0.2382&0.0092&25.8&\textbf{\textless .0001}\tabularnewline
dataset: PTB&0.2923&0.0088&33.38&\textbf{\textless .0001}\tabularnewline
generation x abstract structure: used&-0.0044&7e-04&-6&\textbf{\textless .0001}\tabularnewline
generation x dataset: PTB&0.0042&7e-04&6.03&\textbf{\textless .0001}\tabularnewline
\hline
&&&&\tabularnewline
Random Effects&&&&\tabularnewline
&Std. Dev&&&\tabularnewline
(Intercept) $|$ Recording Chain&0.35&&&\tabularnewline
generation $|$ Recording Chain&0.03&&&\tabularnewline
\bottomrule
\multicolumn{5}{l}{\footnotesize{Note: Significance of fixed-effects is computed following Satterthwaite, 1946.}}
\end{tabular}\end{center}
\end{table}


==> Telephone - Cognition revision 3-2/includes/structureTests_vars.tex <==
\newcommand{\structureTestsIntercept}{($\beta$ = 2.3362, \textit{t} value = 85.81, $p$ $<$ .0001)}
\newcommand{\structureTestsgeneration}{($\beta$ = 0.001, \textit{t} value = 0.38, $p$ = 0.7)}
\newcommand{\structureTestsabstractstructureused}{($\beta$ = 0.2382, \textit{t} value = 25.8, $p$ $<$ .0001)}
\newcommand{\structureTestsdatasetPTB}{($\beta$ = 0.2923, \textit{t} value = 33.38, $p$ $<$ .0001)}
\newcommand{\structureTestsgenerationxabstractstructureused}{($\beta$ = -0.0044, \textit{t} value = -6, $p$ $<$ .0001)}
\newcommand{\structureTestsgenerationxdatasetPTB}{($\beta$ = 0.0042, \textit{t} value = 6.03, $p$ $<$ .0001)}
\newcommand{\structureTestsInterceptRecordingChain}{(Std. Dev. = 0.35}
\newcommand{\structureTestsgenerationRecordingChain}{(Std. Dev. = 0.03}

==> Telephone - Cognition revision 3-2/includes/wordLevel_lm.tex <==
%latex.default(rdf, file = file, title = "", table.env = FALSE,     booktabs = TRUE, ...)%
\begin{table}[t]
\caption{Mixed-effects logistic regression predicting whether a word will be changed in transmission on the basis of its surprisal under various language models as well as other word properties.\label{tab:wordlevel_lm}} 
\begin{center}
\begin{tabular}{lllll}
\toprule
Fixed Effects&&&&\tabularnewline
\multicolumn{1}{l}{}&\multicolumn{1}{c}{Coef $\beta$}&\multicolumn{1}{c}{SE($\beta$)}&\multicolumn{1}{c}{\textit{z} value}&\multicolumn{1}{c}{$Pr(>|\textit{z}|)$}\tabularnewline
\midrule
(Intercept)&-2.6554&0.0933&-28.45&\textbf{\textless .0001}\tabularnewline
BNC unigram surprisal&0.3827&0.0222&17.25&\textbf{\textless .0001}\tabularnewline
Residualized BNC trigram surprisal&0.3729&0.0193&19.37&\textbf{\textless .0001}\tabularnewline
Residualized Roark PCFG syntactic surprisal&0.1159&0.0266&4.36&\textbf{\textless .0001}\tabularnewline
Residualized Big LM surprisal&0.1959&0.0181&10.82&\textbf{\textless .0001}\tabularnewline
Residualized DS 5-gram surprisal&0.1593&0.0262&6.07&\textbf{\textless .0001}\tabularnewline
Position in sentence&0.0989&0.0064&15.57&\textbf{\textless .0001}\tabularnewline
Age of acquisition&0.0544&0.0137&3.96&\textbf{\textless .0001}\tabularnewline
Number of phonemes&-0.0609&0.0231&-2.64&\textbf{\textless .01}\tabularnewline
Number of syllables&-0.249&0.0507&-4.91&\textbf{\textless .0001}\tabularnewline
Concreteness&-0.0856&0.0192&-4.46&\textbf{\textless .0001}\tabularnewline
Phonological Neighborhood Density (PLD20)&-0.0948&0.0427&-2.22&\textbf{\textless .05}\tabularnewline
\hline
&&&&\tabularnewline
Random Effects&&&&\tabularnewline
&Std. Dev.&&&\tabularnewline
\hline
Listener ID&0.62&&&\tabularnewline
Speaker ID&0.3&&&\tabularnewline
\bottomrule
\multicolumn{5}{l}{\footnotesize{Note: Significance of fixed-effects is computed following Satterthwaite, 1946.}}
\end{tabular}\end{center}
\end{table}


==> Telephone - Cognition revision 3-2/includes/wordLevel_vars.tex <==
\newcommand{\wordLevelIntercept}{($\beta$ = -2.6554, \textit{z} value = -28.45, $p$$<$ .0001)}
\newcommand{\wordLevelBNCunigramsurprisal}{($\beta$ = 0.3827, \textit{z} value = 17.25, $p$$<$ .0001)}
\newcommand{\wordLevelResidualizedBNCtrigramsurprisal}{($\beta$ = 0.3729, \textit{z} value = 19.37, $p$$<$ .0001)}
\newcommand{\wordLevelResidualizedRoarkPCFGsyntacticsurprisal}{($\beta$ = 0.1159, \textit{z} value = 4.36, $p$$<$ .0001)}
\newcommand{\wordLevelResidualizedBigLMsurprisal}{($\beta$ = 0.1959, \textit{z} value = 10.82, $p$$<$ .0001)}
\newcommand{\wordLevelResidualizedDSgramsurprisal}{($\beta$ = 0.1593, \textit{z} value = 6.07, $p$$<$ .0001)}
\newcommand{\wordLevelPositioninsentence}{($\beta$ = 0.0989, \textit{z} value = 15.57, $p$$<$ .0001)}
\newcommand{\wordLevelAgeofacquisition}{($\beta$ = 0.0544, \textit{z} value = 3.96, $p$$<$ .0001)}
\newcommand{\wordLevelNumberofphonemes}{($\beta$ = -0.0609, \textit{z} value = -2.64, $p$$<$ .01)}
\newcommand{\wordLevelNumberofsyllables}{($\beta$ = -0.249, \textit{z} value = -4.91, $p$$<$ .0001)}
\newcommand{\wordLevelConcreteness}{($\beta$ = -0.0856, \textit{z} value = -4.46, $p$$<$ .0001)}
\newcommand{\wordLevelPhonologicalNeighborhoodDensity}{($\beta$ = -0.0948, \textit{z} value = -2.22, $p$$<$ .05)}
\newcommand{\wordLevelListenerID}{(Std. Dev. = 0.62}
\newcommand{\wordLevelSpeakerID}{(Std. Dev. = 0.3}
